Repr\'esentations lexicales pour la d\'etection non supervis\'ee d'\'ev\'enements dans un flux de tweets : \'etude sur des corpus fran\c{c}ais et anglais

In this work, we evaluate the performance of recent text embeddings for the automatic detection of events in a stream of tweets. We model this task as a dynamic clustering problem.Our experiments are conducted on a publicly available corpus of tweets in English and on a similar dataset in French annotated by our team. We show that recent techniques based on deep neural networks (ELMo, Universal Sentence Encoder, BERT, SBERT), although promising on many applications, are not very suitable for this task. We also experiment with different types of fine-tuning to improve these results on French data. Finally, we propose a detailed analysis of the results obtained, showing the superiority of tf-idf approaches for this task.

==> contingency.tex <==
\begin{tabular}{|c|c|c|}
\hline
{} & Appartient à l'événement & N'appartient pas à l'événement \\
\hline
Appartient au cluster     &       a &           b \\
\hline
N'appartient pas au cluster &       c &           d \\
\hline
\end{tabular}

